Fragmentation of Transversely Polarized Quarks Probed in Transverse Momentum Distributions

It is shown that the azimuthal dependence of the distribution of hadrons in a quark jet is a probe of the transverse spin of the quark initiating the jet. This results in a new spin-dependent fragmentation function that acts at the twist-2 level. One example of a process where it contributes is semi-inclusive deeply inelastic scattering with a transversely polarized nucleon target but with an {\em unpolarized} electron beam. This process is treated in detail. Another process is the cross section for singly polarized hadron-hadron scattering when two high $p_{\perp}$ hadrons are measured in the final state and are close to back-to-back in azimuth. The new fragmentation function is sensitive to the coupling of the fragmentation process to (spontaneous) chiral symmetry breaking.

==> jccsym.tex <==
% NOT NEEDED FOR TeX 3.14:
% \catcode`\^^?=9%  Cat code for delete => ignore to handle DOS files under UNIX.
%      Math/physics symbols.
%      Revised by J. Collins 21 Oct 93
%
% This file is aimed to be same for both plain TeX and LaTeX.
% For plain TeX, \frac should have been defined earlier.
%

% Use \JCCSYMTEX as flag to prevent processing this file twice
\expandafter \ifx \csname JCCSYMTEX\endcsname \relax
   \def \TMPTMPTMP{}
\else
   \def \TMPTMPTMP{\endinput}
\fi
% If this file has already been processed, (La)TeX will now exit
% this file:
\TMPTMPTMP

\def \JCCSYMTEX {JCCSYMTEX}


%\def\ifundef#1{\expandafter\ifx\csname #1\endcsname\relax}
%\newif \ifLaTeX
%\ifundef{newcommand}\LaTeXfalse \else \LaTeXtrue \fi
%=================================================================
%
%  OBSOLETE:
%
% \def\pr#1{#1^\prime} % OVERRIDDEN BY PHYS REV
%
%=================================================================
%
%
% This defines fractions with appropriate sizes:
%??  Old version: \def\fr#1#2{{\textstyle{#1 \over #2}}}
\def \fr#1#2{\ifinner \innerfr{#1}{#2}  \else \outerfr{#1}{#2}\fi}
\def \innerfr#1#2{\ifmmode \ndmathfr{#1}{#2}
           \else \textfr{#1}{#2}\fi}
\def \outerfr#1#2{\ifmmode \dmathfr{#1}{#2}
           \else \textfr{#1}{#2}\fi}
\def \ndmathfr #1#2{ \raise 0.4 ex\hbox{${\scriptstyle {#1 \over #2}} $} }
\def \dmathfr  #1#2{ {#1 \over #2} }
\def \textfr   #1#2{\raise 0.4 ex\hbox{${\scriptstyle {#1 \over #2}}$}}
%
%
% Sub/superscript preceeding current position:
\def\presbsp#1#2{\hphantom{{}^{#1}_{#2}}
                 \llap{${}^{#1}$} \llap{${}_{#2}$}{}}
%
% Isotope symbol:
\def\iso#1#2#3{\presbsp{#1}{#2} {\rm #3}}
%
%
%=================================================================
%
%
%
\def\la{\mathrel{\mathpalette\fun <}}
\def\ga{\mathrel{\mathpalette\fun >}}
\def\fun#1#2{\lower3.6pt\vbox{\baselineskip0pt\lineskip.9pt
  \ialign{$\mathsurround=0pt#1\hfil##\hfil$\crcr#2\crcr\sim\crcr}}}
%approx less than and greater than
\def\centeron#1#2{{\setbox0=\hbox{#1}\setbox1=\hbox{#2}\ifdim
\wd1>\wd0\kern.5\wd1\kern-.5\wd0\fi
\copy0\kern-.5\wd0\kern-.5\wd1\copy1\ifdim\wd0>\wd1
\kern.5\wd0\kern-.5\wd1\fi}}
%
\def\centerover#1#2{\centeron{#1}{\setbox0=\hbox{#1}\setbox
1=\hbox{#2}\raise\ht0\hbox{\raise\dp1\hbox{\copy1}}}}
%
\def\centerunder#1#2{\centeron{#1}{\setbox0=\hbox{#1}\setbox
1=\hbox{#2}\lower\dp0\hbox{\lower\ht1\hbox{\copy1}}}}
%
%===================================================
%
%     MAIN DEFINITIONS:
%
%----------------These define et al., i.e., e.g., cf., etc:
\def\ie{\hbox{\it i.e.}{}}      \def\etc{\hbox{\it etc.}{}}
\def\eg{\hbox{\it e.g.}{}}      \def\cf{\hbox{\it cf.}{}}
\def\etal{\hbox{\it et al.}}
\def\dash{\hbox{---}}
\def\order {{\cal O}}
%
%----------------Units:  ====
%  Some have Greek in them, so swithc to mathmode if needed:
\def \UNIT #1{{\ifmmode \UNITBODY {#1} \else $ \UNITBODY {#1} $\fi }}
\def \UNITBODY #1{\,{\rm #1}}
\def \MeV {\UNIT{MeV}}
\def \GeV {\UNIT{GeV}}
\def \TeV {\UNIT{TeV}}
% Use \barn, \pbarn to avoid conflict with LaTeX.
\def \barn  {\UNIT{b}}
\def \pbarn  {\UNIT{pb}}
\def \nbarn  {\UNIT{nb}}
\def \mubarn {\UNIT{\mu b}}
\def \mbarn  {\UNIT{mb}}
\def \fm  {\UNIT{fm}}
\def \mm  {\UNIT{mm}}
\def \cm  {\UNIT{cm}}
\def \m   {\UNIT{m}}
\def \mug {\UNIT{\mu g}}
\def \mg  {\UNIT{mg}}
\def \gm  {\UNIT{gm}}
\def \kg  {\UNIT{kg}}
\def \s   {\UNIT{s}}
\def \yr  {\UNIT{yr}}
%
%------------Common physics symbols
\def \al {\alpha_{\rm s}}
\def \alpi {{\alpha_s \over \pi}}
\def \degree {^\circ }
\def \disc{\mathop{\rm disc}}
% \def \dot{{\cdot}}
\def \tr{\mathop{\rm tr}}
\def \Tr{\mathop{\rm Tr}}
\def \T#1{{\bf #1}}% transverse vector
\def \Im{\mathop{\rm Im}}
%\def \MSbar {\vbox{\hrule\kern 1pt\hbox{\rm MS}}}
\def \MSbarbasic {\overline{{\rm MS}}}
\def \MSbar {\ifmmode \MSbarbasic \else $\MSbarbasic$\fi }
\def \Re{\mathop{\rm Re}}
\def \bR{\mathop{\bf R}{}}
\def \bC{\mathop{\bf C}{}}
\def \Lie{\mathop{\cal L}}      % fancy L for the Lie derivative
%       The command \st (for stroke) puts a slash through the succeeding
%       character in math mode
\def \st#1{\centeron{$#1$}{$/$}}
\def \partder#1#2{{\partial #1\over\partial #2}}
\def \secder#1#2#3{{\partial^2 #1\over\partial #2 \partial #3}}
\def \bra#1|{\mathopen{\langle#1\,|}}  %Dirac bra arg. is placed in bra symbol
\def \braket#1|#2>{\langle#1\,|\,#2\rangle} %Dirac braket arg's in bra & ket
\def \ket#1>{\mathclose{|\,#1\rangle}}  %Dirac ket arg. is placed in ket symbol
\def \VEV#1{\left\langle #1\right\rangle}
\def \dalem{\vbox {\hrule height 0.6pt\hbox{\vrule width 0.6pt\hskip 3pt
\vbox{\vskip 6pt}\hskip 3pt \vrule width 0.6pt}\hrule height 0.6pt}}
\def \gdot#1{\rlap{$#1$}/}
\def \abs#1{\left| #1\right|}
\def \ltap{\;\centeron{\raise.35ex\hbox{$<$}}{\lower.65ex\hbox{$\sim$}}\;}
\def \gtap{\;\centeron{\raise.35ex\hbox{$>$}}{\lower.65ex\hbox{$\sim$}}\;}
\def \gsim{\mathrel{\gtap}}
\def \lsim{\mathrel{\ltap}}
\def \simless{\lsim }
\def \cosh{\mathop{\rm cosh}}
\def \d{\,{\rm d}}
\def \diff{\d}
\def \e{{\rm e}}
\def \epem{{\ifmmode \epembody \else $ \epembody $\fi }}
%  Allow correct size in sub and super.
\def \epembody{ \e^+\e^- }
\def \half{\fr12}
\def \p{{\rm p}}
\def \K{{\rm K}}
\def \n{{\rm n}}
\def \N{{\rm N}}
\def \P{{\rm P}}
%
%------------------Journals:
\def \rf    #1#2#3{#1, #2 (19#3)}
\def \jour  #1{#1\ \relax}
\def \rfj   #1#2#3#4{\jour {#1}\rf {#2}{#3}{#4}}
\def \aj    {\jour {Astrophys.\ J.}}
\def \raj   #1#2#3{\rfj {\aj}{#1}{#2}{#3}}
\def \arnps {\jour {Ann.\ Rev.\ Nucl.\ Part. Sci.}}
\def \rarnps#1#2#3{\rfj {\arnps}{#1}{#2}{#3}}
\def \np    {\jour {Nucl.\ Phys.}}
\def \rnp   #1#2#3{\rfj {\np}{#1}{#2}{#3}}
\def \pl    {\jour {Phys.\ Lett.}}
\def \rpl   #1#2#3{\rfj {\pl}{#1}{#2}{#3}}
\def \pr    {\jour {Phys.\ Rev.}}
\def \rpr   #1#2#3{\rfj {\pr}{#1}{#2}{#3}}
\def \prpt  {\jour {Phys.\ Reports}}
\def \rprpt #1#2#3{\rfj {\pr}{#1}{#2}{#3}}
\def \prl   {\jour {Phys.\ Rev.\ Lett.}}
\def \rprl  #1#2#3{\rfj {\prl}{#1}{#2}{#3}}
\def \sjnp  {\jour {Sov.\ J. Nucl.\ Phys.}}
\def \rsjnp #1#2#3{\rfj {\sjnp}{#1}{#2}{#3}}
\def \zphc  {\jour {Z.\ Phys.\ C}}
\def \rzphc #1#2#3{\rfj {\zphc}{#1}{#2}{#3}}
\relax

